Towards Stable and Efficient Training of Verifiably Robust Neural Networks

Training neural networks with verifiable robustness guarantees is challenging. Several existing approaches utilize linear relaxation based neural network output bounds under perturbation, but they can slow down training by a factor of hundreds depending on the underlying network architectures. Meanwhile, interval bound propagation (IBP) based training is efficient and significantly outperforms linear relaxation based methods on many tasks, yet it may suffer from stability issues since the bounds are much looser especially at the beginning of training. In this paper, we propose a new certified adversarial training method, CROWN-IBP, by combining the fast IBP bounds in a forward bounding pass and a tight linear relaxation based bound, CROWN, in a backward bounding pass. CROWN-IBP is computationally efficient and consistently outperforms IBP baselines on training verifiably robust neural networks. We conduct large scale experiments on MNIST and CIFAR datasets, and outperform all previous linear relaxation and bound propagation based certified defenses in $\ell_\infty$ robustness. Notably, we achieve 7.02% verified test error on MNIST at $\epsilon=0.3$, and 66.94% on CIFAR-10 with $\epsilon=8/255$. Code is available at https://github.com/deepmind/interval-bound-propagation (TensorFlow) and https://github.com/huanzhang12/CROWN-IBP (PyTorch).

==> big_table_new.tex <==
\newcolumntype{g}{>{\columncolor{Gray}}c}
\begin{table}[t!]
\centering
    \caption{The verified and standard (clean) test errors for 3 models (small, medium, large) trained on MNIST and CIFAR. We evaluate IBP and CROWN-IBP under different $\kappa$ schedules. CROWN-IBP outperforms IBP under the same $\kappa$ setting, and also achieves state-of-the-art results for $\ell_\infty$ robustness on both MNIST and CIFAR datasets for all $\epsilon$.
    \sven{For consistency, I'd top-align the 3rd to last column. (Done.)}
    \todo{make text larger, probably move small/medium to appendix, also report PGD (important!)}}
    \label{tbl:three_model_result} 
\adjustbox{max width=1.00\linewidth}{
\begin{threeparttable}
    \begin{tabular}{c!{\vrule width 1.3pt}c!{\vrule width 1.3pt}c!{\vrule width 1.3pt}c|c!{\vrule width 1.3pt}c|g!{\vrule width 1.3pt}c|g!{\vrule width 1.3pt}c|g!{\vrule width 1.3pt}c!{\vrule width 1.3pt}c|c|g}
    \toprule[2pt]
        Dataset & $\epsilon$ ($\ell_\infty$ norm) & Training Method & \multicolumn{2}{c!{\vrule width 1.3pt}}{$\kappa$ schedules}   & \multicolumn{2}{c!{\vrule width 1.3pt}}{\textbf{Small} model's err. (\%)} & \multicolumn{2}{c!{\vrule width 1.3pt}}{\textbf{Medium} model's err. (\%)}  &\multicolumn{2}{c!{\vrule width 1.3pt}}{\textbf{Large} model's err. (\%)} &  & \multicolumn{3}{c}{\textbf{Best} errors reported in literature (\%)} \\
        
        & & & $\kappa_\text{start}$&$\kappa_\text{end}$ & \ Standard\   &\textbf{Verified} &\ \ \ Standard\ \ \  &\textbf{Verified} & \ Standard\   & \textbf{Verified} && Source & Standard & \textbf{Verified} \\ 
        \midrule[1.5pt]
      \multirow{30}{*}{\shortstack{MNIST}} &   & \multirow{3}{*}{IBP}&0&0 &  1.92	&	4.16  &1.53	&	3.26&1.13	&	2.89&  & \multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{$1.06$}& \multirow{1}{*}{$2.92$\tnote{1}} \\
       &   & & 1&0.5 &    1.68	&	3.60  & 1.46	&	3.20&1.08	&	2.75&&\multirow{1}{*}{\cite{dvijotham2018training}}&\multirow{1}{*}{1.2}& \multirow{1}{*}{4.44}\\
       &  $\epsilon_\text{test}=0.1$ & & 1&0 &    2.14	&	4.24&1.48	&	3.21&1.14	&	2.81  & &\multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{$1.05$}& \multirow{1}{*}{$4.4$} \\
       
    %   \midrule
    \cline{3-11}
 
    
        & \multirow{1}{*}{$\epsilon_\text{train}= 0.2$}& \multirow{3}{*}{CROWN-IBP} &0&0 &  1.90	&	3.05&1.44	&	2.77  & 1.17	&	2.36 & & \multirow{1}{*}{\cite{wong2018scaling}}&\multirow{1}{*}{1.08}& \multirow{1}{*}{3.67} \\
       &   & & 1&0.5 &    1.60	&	3.51&   1.14	&	\textbf{2.64}&0.95	&	2.38 & &\multirow{1}{*}{\cite{mirman2018differentiable}}&\multirow{1}{*}{1.0}& \multirow{1}{*}{3.4} \\
       &   & & 1&0 &    1.67	&	\textbf{3.44}&1.34	&	2.76&1.17	&	\textbf{2.24}    & &&& \\
    %   \midrule
    \cmidrule[1.5pt]{2-15}
    
    
    &    & \multirow{3}{*}{IBP}&0&0 & 5.08	&	9.80& 3.68	&	7.38&3.50	&	6.56&   &\multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{$1.66$}& \multirow{1}{*}{$4.53$\tnote{1}} \\
       &   & & 1&0.5 &    3.83	&	8.64& 2.55	&	5.84& 2.30	&	5.47&& \multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{$1.9$}& \multirow{1}{*}{$10.21$}\\
       &  $\epsilon_\text{test}= 0.2$ & & 1&0 &    6.25	&	11.32&3.89	&	7.21& 2.60	&	5.70&&&&\\
       
    %   \midrule
    \cline{3-11}
 
    
        & \multirow{1}{*}{$\epsilon_\text{train}= 0.4$}& \multirow{3}{*}{CROWN-IBP} &0&0 &      3.78& 6.61&  3.84& 6.65& 2.84& 5.15& &&&\\
       &   & & 1&0.5 &     2.96& \textbf{6.11}&2.37& \textbf{5.35}&   1.82& \textbf{4.13}& &&& \\
       &   & & 1&0 &      3.55& 6.29&3.16& 5.82& 2.17& 4.31&& & &\\
       
    %   \midrule
    \cmidrule[1.5pt]{2-15}
       
       

       
       
    &    & \multirow{3}{*}{IBP}&0&0 &   5.08	&	14.42& 3.68	&	10.97  & 3.45	&	9.76 & &\multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{1.66}&\multirow{1}{*}{8.21\tnote{1}}\\
       &   & & 1&0.50 &      3.83	&	13.99& 2.55	&	9.51&2.12	&	8.47 & & \multirow{1}{*}{\cite{wong2018scaling}}&\multirow{1}{*}{14.87}&\multirow{1}{*}{43.1}\\
       & $\epsilon_\text{test}= 0.3$  & & 1&0 &      6.25	&	16.51& 3.89	&	10.4&2.74	&	8.73 & & \multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{2.67}&\multirow{1}{*}{19.32}\\
       
    %   \midrule
    \cline{3-11}
 
    
%        & \multirow{1}{*}{$\epsilon_\text{train}= 0.33$}& \multirow{3}{*}{CROWN-IBP} &0&0 &     2.91& 9.51&  2.43& 8.90& 1.73& 7.46&&& & \\
%       &   & & 1&0.5 &      2.15& \textbf{9.26}& 1.61& 8.65& 1.36& 7.65& &&&\\
%       &   & & 1&0 &      2.61& 8.71& 2.17& \textbf{8.53}&1.58& \textbf{7.40} &&\multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{2.67}&\multirow{1}{*}{19.32}\\
      
    %   \midrule
%    \cmidrule[1.5pt]{2-15}
%       
%        
%       
%       
%       
%       
%    &    & \multirow{3}{*}{IBP}&0&0&     3.82& 11.29& 6.97& 15.92&4.56& 11.26& %&\multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{1.66}&\multirow{1}{*}{8.21\tnote{1}}\\
%       &   & & 1&0.5&      3.67& 12.99& 2.68& 9.86&2.31& 9.18& & & &\\
%       &  $\epsilon_\text{test}= 0.3$ & & 1&0 &      4.66& 12.72& 3.66& 10.32&3.04& 9.71&& %\multirow{1}{*}{\cite{wong2018scaling}}&\multirow{1}{*}{14.87}&\multirow{1}{*}{43.1}\\
       
    %   \midrule
    \cline{3-11}
 
    
        & \multirow{1}{*}{$\epsilon_\text{train}= 0.4$}& \multirow{3}{*}{CROWN-IBP} &0&0 &      3.78& 9.60& 3.84& 9.25& 2.84& 7.65& &&&\\
       &   & & 1&0.5 &      2.96& 9.44&   2.37& \textbf{8.54}& 1.82&\textbf{ 7.02}&  &&&\\
       &   & & 1&0 &      3.55&\textbf{ 9.40}&  3.16& 8.62&  2.17& 7.03&&&&\\
       
       \cmidrule[1.5pt]{2-15}
       
        
       
       
       
       
    &    & \multirow{3}{*}{IBP}&0&0&      5.08	&	23.4& 3.68	&	18.34&  3.45	&	16.19&  &\multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{1.66}&\multirow{1}{*}{15.01\tnote{1}}\\
       &   & & 1&0.5&      3.83	&	24.16& 2.55	&	16.82&2.12	&	15.37& & & &\\
       &  $\epsilon_\text{test}= 0.4$ & & 1&0 &      6.25	&	26.81& 3.89	&	16.99&  2.74	&	14.8& &&&\\
       
    %   \midrule
    \cline{3-11}
 
    
        & \multirow{1}{*}{$\epsilon_\text{train}= 0.4$}& \multirow{3}{*}{CROWN-IBP} &0&0 &      3.78& \textbf{15.21}& 3.84& 14.58& 2.84& 12.74
& &&&\\
       &   & & 1&0.5 &      2.96& 16.04& 2.37& 14.97& 1.82& 12.59& & & &\\
       &   & & 1&0 &      3.55& 15.55&  3.16& \textbf{14.19}&  2.17& \textbf{12.06}&&& &\\
       

    
       

    
        \midrule[1.5pt]
    \multirow{18}{*}{\shortstack{CIFAR-10}} &    & \multirow{3}{*}{IBP}&0&0 &      44.66	&	56.38	&39.12& 53.86&38.54& 55.21  & &\multirow{1}{*}{\cite{mirman2018differentiable}}&\multirow{1}{*}{38.0}&\multirow{1}{*}{47.8}\\
       &   & & 1&0.5 &      38.90	&	57.94	&34.19& 56.24  &33.77& 58.48&& \multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{29.84}&\multirow{1}{*}{55.88\tnote{1}}\\
       & $\epsilon_\text{test}= 2/255$  & & 1&0 &      44.08	&	56.32	&39.30& 53.68  &39.22& 55.19& & \multirow{1}{*}{\cite{wong2018scaling}}&\multirow{1}{*}{31.72}&\multirow{1}{*}{46.11}\\
       
    %   \midrule
    \cline{3-11}
 
    
        & \multirow{1}{*}{$\epsilon_\text{train}= 2.2/255$\tnote{3}}& \multirow{3}{*}{CROWN-IBP} &0&0 &    39.43	&	53.93	&32.78	&	\textbf{49.57}	&28.48	&	\textbf{46.03}	& &\multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{38.88}&\multirow{1}{*}{54.07}\\
       &   & & 1&0.5 &      34.08	&	54.28	& 28.63	&	51.39	&26.19	&	50.53	& &&&\\
       &   & & 1&0 &      38.15	&	\textbf{52.57}	&33.17	&	49.82	&28.91	&	46.43	& &&&\\
       
    %   \midrule
    \cmidrule[1.5pt]{2-15}
    
    
    &    & \multirow{3}{*}{IBP}&0&0 &   61.91	&	73.12	&61.46& 71.98 &59.41& 71.22  &   & \multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{50.51}&\multirow{1}{*}{(68.44\tnote{2}\enskip)}\\
       &   & & 1&0.5 &      54.01	&	73.04	&50.33& 73.58 & 49.01& 72.68& & \multirow{1}{*}{\cite{dvijotham2018training}}&\multirow{1}{*}{51.36}&\multirow{1}{*}{73.33}\\
       &  $\epsilon_\text{test}= 8/255$ & & 1&0 &      62.66	&	72.25	&61.61& 72.60 & 58.43& 70.81& &\multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{59.55}&\multirow{1}{*}{79.73}\\
       
    %   \midrule
    \cline{3-11}
 
    
        & \multirow{1}{*}{$\epsilon_\text{train}= 8.8/255$\tnote{3}}& \multirow{3}{*}{CROWN-IBP} &0&0 &      59.94	&	70.76	&59.17& 69.00 &54.02& \textbf{66.94} & &\multirow{1}{*}{\cite{wong2018scaling}}&\multirow{1}{*}{71.33}&\multirow{1}{*}{78.22}\\
       &   & & 1&0.5 &      53.12	&	73.51	&48.51& 71.55  &45.47& 69.55 & && &\\
       &   & & 1&0 &      58.19& \textbf{68.94} & 55.21& \textbf{68.14}&55.27& 67.76& &&&\\
       
    %   \midrule
    
    \cmidrule[1.5pt]{2-15}
    
    
    &    & \multirow{3}{*}{IBP}&0&0 &   70.02	&	78.86	&67.55& 78.65 &68.97& 78.12  &   & \multicolumn{3}{c}{\multirow{6}{*}{\makecell{None, but our best verified test error (76.80\%)\\and standard test error (66.06\%) are both better\\ than~\cite{wong2018scaling} at $\epsilon=\frac{8}{255}$, despite our\\ $\epsilon$ being twice larger.}}}\\
       &   & & 1&0.5 &      63.43	&	81.58	&60.07& 81.01 & 59.46& 80.85& &\multicolumn{3}{c}{}\\
       &  $\epsilon_\text{test}= 16/255$ & & 1&0 &      67.73	&	78.71	&70.28& 79.26 & 68.88& 78.91& &\multicolumn{3}{c}{}\\
       
    %   \midrule
    \cline{3-11}
 
    
        & \multirow{1}{*}{$\epsilon_\text{train}= 17.6/255$\tnote{3}}& \multirow{3}{*}{CROWN-IBP} &0&0 &      67.42	&	\textbf{78.41}	&68.06& 77.92 &67.17& 77.27 & &\multicolumn{2}{c}{}\\
       &   & & 1&0.5 &      61.47	&	79.62	&59.56& 79.30  &56.73& 78.20 & &\multicolumn{2}{c}{}\\
       &   & & 1&0 &      68.75	&	78.71	&67.94&\textbf{78.46} &66.06& \textbf{76.80}& &\multicolumn{2}{c}{}\\
       
    %   \midrule

    \bottomrule[2pt]
    \end{tabular}
\begin{tablenotes}
\linespread{1.5}\selectfont

\item[1] {\Large Verified errors reported in Table 4 of \cite{gowal2018effectiveness} are evaluated using mixed integer programming (MIP). For a fair comparison, we use the IBP verified errors reported in Table 3 of \cite{gowal2018effectiveness}.
}
\item[2] {\Large According to direct communication with the authors of~\cite{gowal2018effectiveness}, achieving 68.44\% IBP verified error requires to adding an extra PGD adversarial training loss. Without adding PGD, the achievable verified error is 72.91\% (LP/MIP verified) or 73.52\% (IBP verified).
}
\item[3] {\Large Although not explicitly mentioned, the best CIFAR-10 models in~\citep{gowal2018effectiveness} also use $\epsilon_{\text{train}}=1.1\epsilon_{\text{test}}$.}

\end{tablenotes}
    \end{threeparttable}
}
%
    % \captionof{table}{Untargeted attack success rate against Mitsuba by transferring ``adversarial meshes'' generated by attacking a differentiable renderer targeting different classes.}
    %\vspace{-0.5cm}
\end{table}

==> bigtable1_before.tex <==
%\vspace{-0.5cm}
\begin{table}[ht!]
\centering
    \caption{The verified and standard (clean) test errors for models trained on MNIST, Fashion-MNIST and CIFAR using different methods. Here we train 53 models using CROWN-IBP, and IBP with different $\kappa_\text{start}$ and $\kappa_\text{end}$. For each training method, we pick 3 representative models among all models: the models with smallest, median, and largest verified error. We also report the standard error of \emph{these three selected models}. }%\textcolor{blue}{the table looks like we only have 2 models, one large and one small. We should make sure other people do not misunderstand us.}
    \label{tbl:result} 
\adjustbox{max width=1.00\linewidth}{
\begin{threeparttable}
    \begin{tabular}{c!{\vrule width 1.3pt}c!{\vrule width 1.3pt}c!{\vrule width 1.3pt}c!{\vrule width 1.3pt}c|c!{\vrule width 1.3pt}g|g|g!{\vrule width 1.3pt}c|c|c!{\vrule width 1.3pt}c!{\vrule width 1.3pt}c|g|c}
    \toprule[2pt]
        Dataset & $\epsilon$ ($\ell_\infty$ norm) & Model Family & Training Method&\multicolumn{2}{c!{\vrule width 1.3pt}}{$\kappa$ schedule}   & \multicolumn{3}{c!{\vrule width 1.3pt}}{ Verified Test Error (\%)}& \multicolumn{3}{c!{\vrule width 1.3pt}}{ Standard Test Error(\%)} &  & \multicolumn{3}{c}{\textbf{Best} results reported in literature (\%)} \\
        
        & & & &$\kappa_\text{start}$ &$\kappa_\text{end}$& best &median& worst & best & median & worst & & Source & Verified Err. & Std. Err. \\ 
        \midrule[1.5pt]
      \multirow{48}{*}{\shortstack{MNIST}} &    & \multirow{6}{*}{10 small models}&\multirow{3}{*}{IBP}&0&0 & 4.79 & 5.74 & 7.32 & 1.48 & 1.59 & 2.5 & & \multirow{1}{*}{\cite{gowal2018effectiveness}}& \multirow{1}{*}{$2.23$\tnote{1}}&\multirow{1}{*}{$1.06$} \\
       &   & && 1&0 &4.87 & 5.72 & 7.24 & 1.51 & \textbf{1.34} & 2.46 & & \multirow{1}{*}{\cite{xiao2018training}}& \multirow{1}{*}{$4.4$}&\multirow{1}{*}{$1.05$}\\
       &   & && 1&0.5 &5.24 & 5.95 & 7.36 & 1.41 & 1.88 & \textbf{1.87} & &\multirow{1}{*}{\cite{mirman2018differentiable}}& \multirow{1}{*}{3.4}&\multirow{1}{*}{1.0} \\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0&\textbf{4.21}\tnote{1} & \textbf{5.18} & \textbf{6.8} & \textbf{1.41} & 1.83 & 2.58& & \multirow{1}{*}{\cite{wong2018scaling}}& \multirow{1}{*}{3.67}&\multirow{1}{*}{1.08}\\
       &    &   &   & 1  & 0  &  4.14   & 5.24  & 6.82  &1.39 & 2.06  &  2.46 &   &  \multirow{1}{*}{\cite{dvijotham2018training}}& \multirow{1}{*}{4.44}&\multirow{1}{*}{1.2}   \\
       &  $\epsilon_\text{train}=0.1$\tnote{1}  &   &   & 1  & 0.5  &  4.62 &  5.94 & 6.88  & 1.26  & 1.88  &  1.97 &   &  &   &   \\
    %   \midrule
    \cline{3-12}
 
    
        &$\epsilon_\text{test}=0.1$ & \multirow{6}{*}{8 medium models} &\multirow{3}{*}{IBP}&0&0 & 5.9 & 6.25 & 7.82 & \textbf{1.14} & 1.12 & 1.23& & && \\
       &   & && 1&0 & 5.77 & 6.30 & 7.50 & 1.21 & 1.13 & 1.34 & & && \\
       &   & && 1&0.5 & 6.05 & 6.40 & 7.70 & 1.19 & 1.33 & 1.24 & &&& \\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0& \textbf{5.22}\tnote{1} & \textbf{5.63} & \textbf{6.34} & 1.19 & \textbf{1.05} & \textbf{1.03} & &&&\\
       &    &   &   &  1 & 0  & 5.43  &  5.90 & 6.02  & 1.30  & 1.03  & 1.09  &   &  &   &   \\
       &    &   &   &  1 &  0.5 & 5.44  & 5.89  & 6.09  &  1.11 & 1.16  & 1.01  &   &  &   &   \\
    %   \midrule
    \cmidrule[1.5pt]{2-16}
    
    
    &    & \multirow{6}{*}{10 small models}&\multirow{3}{*}{IBP}&0&0 & 6.9 & 8.24 & 12.67 & 1.93 & 2.76 & 4.14 & &\multirow{1}{*}{\cite{gowal2018effectiveness}}& \multirow{1}{*}{$4.48$\tnote{2}}&\multirow{1}{*}{$1.66$} \\
       &   & && 1&0 & 6.84 & 8.16 & 12.92 & 2.01 & 2.56 & 3.93 & & \multirow{1}{*}{\cite{xiao2018training}}& \multirow{1}{*}{$10.21$}&\multirow{1}{*}{$1.9$} \\
       &   & && 1&0.5 &7.31 & 8.71 & 13.54 & \textbf{1.62} & 2.36 & \textbf{3.22} & &&&\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0&\textbf{6.11}\tnote{1} & \textbf{7.29} & \textbf{11.97} & 1.93 & \textbf{2.3} & 3.86 & & & &\\
       &    &   &   &  1 & 0  & 6.27  & 7.66  &  12.11 & 2.01  & 2.92  & 4.06  &   &  &   &   \\
       &  $\epsilon_\text{train}=0.2$\tnote{1}  &   &   &  1 &  0.5 & 6.53  & 8.14  &  12.56 &  1.61 &  1.61 & 3.27  &   &  &   &   \\
    %   \midrule
    \cline{3-12}
 
    
        &$\epsilon_\text{test}=0.2$ & \multirow{6}{*}{8 medium models} &\multirow{3}{*}{IBP}&0&0 & 7.56 & 8.6 & 9.8 & 1.96 & 2.19 & 1.39 & &&&\\
       &   & && 1&0 &8.26 & 8.72 & 9.84 & 1.45 & 1.73 & \textbf{1.31} & & & &\\
       &   & && 1&0.5 & 8.42 & 8.9 & 10.09 & 1.76 & 1.42 & 1.53 & & & &\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0& \textbf{6.06}\tnote{1} & \textbf{6.42} & \textbf{7.64} & \textbf{1.09} & \textbf{1.33} & 1.36 & & & &\\
       &    &   &   &  1 & 0  & 6.39  & 7.09  & 7.84  & 1.11  &  1.04 & 1.25  &   &  &   &   \\
       &    &   &   &  1 &  0.5 & 6.63  & 7.51  & 7.96  &  1.08 & 1.25&  1.19   &   &  &   &   \\
    %   \midrule
    \cmidrule[1.5pt]{2-16}
       
       

       
       
    &    & \multirow{6}{*}{10 small models}&\multirow{3}{*}{IBP}&0&0 & 10.54 & 12.02 & 20.47 & 2.78 & \textbf{3.31} & 6.07 & &\multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{8.05\tnote{1}}&\multirow{1}{*}{1.66}\\
       &   & && 1&0 &9.96 & 12.09 & 21.0 & 2.7 & 3.48 & 6.68 & &\multirow{1}{*}{\cite{wong2018scaling}}&\multirow{1}{*}{43.1}&\multirow{1}{*}{14.87}\\
       &   & && 1&0.5 & 10.37 & 12.78 & 21.99 & \textbf{2.11} & 3.44 & \textbf{5.19}& & \multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{19.32}&\multirow{1}{*}{2.67}\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0& \textbf{8.87} & \textbf{11.29} & \textbf{16.83} & 2.43 & 3.62 & 7.26 & & &&\\
       &    &   &   &  1 & 0  & 9.69  & 11.33  &  15.23 &  2.78 &  3.41 & 5.90  &   &  &   &   \\
       &  $\epsilon_\text{train}=0.3$  &   &   &  1 &  0.5 & 9.90  & 11.98  &  19.56 & 2.20  & 2.72  & 4.83  &   &  &   &   \\
    %   \midrule
    \cline{3-12}
 
    
        &$\epsilon_\text{test}=0.3$ & \multirow{6}{*}{8 medium models} &\multirow{3}{*}{IBP}&0&0 & 10.43 & 10.83 & 11.99 & 2.01 & 2.38 & 3.29 & & & & \\
       &   & && 1&0 & 10.74 & 11.73 & 12.16 & 2.17 & 2.46 & \textbf{1.6} & &&&\\
       &   & && 1&0.5 & 11.23 & 11.71 & 12.4 & 1.72 & 2.09 & 1.63 & & & &\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0&\textbf{7.46} & \textbf{8.47} & \textbf{8.57} & \textbf{1.48} & \textbf{1.52} & 1.99 & & & &\\
       &    &   &   &  1 & 0  & 7.96  & 8.53  &  8.99 & 1.45  &  1.56 & 1.85  &   &  &   &   \\
       &    &   &   &  1 &  0.5 & 8.19  & 9.20  & 9.51  & 1.27  & 1.46  & 1.62  &  &   &   \\
    %   \midrule
    \cmidrule[1.5pt]{2-16}
       
        
       
       
       
       
    &    & \multirow{6}{*}{10 small models}&\multirow{3}{*}{IBP}&0&0& 16.72 & 18.89 & 37.42 & 4.2 & 5.4 & 9.63 & &\multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{14.88}&\multirow{1}{*}{1.66}\\
       &   & && 1&0 & 16.1 & 18.75 & 35.3 & 3.8 & 4.93 & 11.32 & & & &\\
       &   & && 1&0.5 & 16.54 & 19.14 & 35.42 & \textbf{3.4} & \textbf{3.65} & \textbf{7.54} & & & &\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0&\textbf{15.38} & \textbf{18.57} & \textbf{24.56} & 3.61 & 4.83 & 8.46 & & & &\\
       &    &   &   &  1 & 0  & 16.22  & 18.20  & 24.80  & 4.23  & 5.15  &  8.54 &   &  &   &   \\
       &  $\epsilon_\text{train}=0.4$  &   &   &  1 &  0.5 & 15.97  & 19.18  &  24.76 & 3.48  & 3.97  & 6.64  &   &  &   &   \\
    %   \midrule
    \cline{3-12}
 
    
        &$\epsilon_\text{test}=0.4$ & \multirow{6}{*}{8 medium models} &\multirow{3}{*}{IBP}&0&0 & 15.17 & 16.54 & 18.98 & 2.83 & 3.79 & 4.91 &&&&\\
       &   & && 1&0 &15.63 & 16.06 & 17.11 & 2.93 & 3.4 & 3.75 & & & &\\
       &   & && 1&0.5 & 15.74 & 16.42 & 17.98 & \textbf{2.35} & \textbf{2.31} & \textbf{3.15} & & & &\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0&\textbf{12.96} & \textbf{13.43} & \textbf{14.25} & 2.76 & 2.85 & 3.36 & & & &\\
       &    &   &   &  1 & 0  & 12.90  & 13.47  & 14.06  &  2.42 & 2.86  &  3.11 &   &  &   &   \\
       &    &   &   &  1 &  0.5 & 13.02  & 13.69  &  14.52 & 1.89  & 2.40  & 2.35  &   &  &   &   \\

    \midrule[1.5pt]
    
    % Fashion-MNIST
        \multirow{12}{*}{\shortstack{Fasthion-MNIST}} &    & \multirow{6}{*}{10 small models}&\multirow{3}{*}{IBP}&0&0& 22.91 &23.92 &\textbf{25.70} &16.14 &16.23 &18.66 & &\multirow{1}{*}{\cite{wong2018provable}}&\multirow{1}{*}{34.53}&\multirow{1}{*}{21.73}\\
       &   & && 1&0 & 22.34 &23.72 &25.43 &15.10 &16.22 &17.65 & & & &\\
       &   & && 1&0.5 &23.44 &24.62 &26.21 &\textbf{13.20} &\textbf{14.58} &\textbf{15.02}& & & &\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0&\textbf{22.00} &\textbf{23.43} &25.87 &15.11 &16.44 &18.08 & & & &\\
       &    &   &   &  1 & 0  &   &   &   &   &   &   &   &  &   &   \\
       &  $\epsilon_\text{train}=0.1$  &   &   &  1 &  0.5 &   &   &   &   &   &   &   &  &   &   \\
    %   \midrule
    \cline{3-12}
 
    
        &$\epsilon_\text{test}=0.1$ & \multirow{6}{*}{8 medium models} &\multirow{3}{*}{IBP}&0&0 & 22.37 &23.01 &23.73 &15.57 &15.43 &15.25 &&&&\\
       &   & && 1&0 &22.07 &23.74 &25.56 &14.82 &13.95 &15.31 & & & &\\
       &   & && 1&0.5 & 23.87 &25.47 &27.19 &12.72 &\textbf{13.62} &\textbf{13.07} & & & &\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0&\textbf{21.27} &\textbf{21.71} &\textbf{22.43} &\textbf{14.19} &14.70 &15.41 & & & &\\
       &    &   &   &  1 & 0  &   &   &   &   &   &   &   &  &   &   \\
       &    &   &   &  1 &  0.5 &   &   &   &   &   &   &   &  &   &   \\

    \midrule[1.5pt]
    
    \multirow{24}{*}{\shortstack{CIFAR-10}} &    & \multirow{6}{*}{9 small models}&\multirow{3}{*}{IBP}&0&0 & 54.69 & 57.84 & 60.58 & 40.59 & 45.51 & 51.38 & &\multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{49.98}&\multirow{1}{*}{29.84}\\
       &   & && 1&0 & 54.56 & 58.42 & 60.69 & 40.32 & 47.42 & 50.73 & & \multirow{1}{*}{\cite{mirman2018differentiable}}&\multirow{1}{*}{47.8}&\multirow{1}{*}{38.0}\\
       &   & && 1&0.5 & 56.89 & 60.66 & 63.58 & \textbf{34.28} & \textbf{39.28} & \textbf{48.03}& & \multirow{1}{*}{\cite{wong2018scaling}}&\multirow{1}{*}{46.11}&\multirow{1}{*}{31.72}\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0& \textbf{52.46} & \textbf{57.55} & \textbf{60.67} & 39.11 & 46.76 & 50.86 & & \multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{54.07}&\multirow{1}{*}{38.88}\\
       &    &   &   &  1 & 0  &  53.62 & 57.52  &  61.01 & 38.23  & 46.17  & 52.22  &   &  &   &   \\
       &  $\epsilon_\text{train}=2/255\tnote{3}$  &   &   &  1 &  0.5 & 56.66  & 60.51  & 63.48  & 34.11  &  41.37 & 47.66  &   &  &   &   \\
    %   \midrule
    \cline{3-12}
 
    
        & $\epsilon_\text{test}=2/255$& \multirow{6}{*}{8 medium models} &\multirow{3}{*}{IBP}&0&0 & 55.47 & 56.41 & 58.54 & 41.59 & 44.33 & 46.54 & &&&\\
       &   & && 1&0 & 55.51 & 56.74 & 57.85 & 42.41 & 43.71 & 44.74 & &&&\\
       &   & && 1&0.5 & 57.05 & 59.7 & 60.25 & \textbf{34.77} & \textbf{35.8} & \textbf{38.95} & &&&\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0& \textbf{52.52} & \textbf{53.9} & \textbf{56.05} & 39.34 & 40.07 & 43.57 & & & &\\
       &    &   &   &  1 & 0  &  53.35 & 54.60  & 57.06  & 38.50  & 40.78  & 43.58  &   &  &   &   \\
       &    &   &   &  1 &  0.5 &  56.04 & 57.34  &60.57   & 32.86  &  34.48 & 38.89  &   &  &   &   \\
    %   \midrule
    \cmidrule[1.5pt]{2-16}
    
    
    &    & \multirow{6}{*}{9 small models}&\multirow{3}{*}{IBP}&0&0 & 72.07 & 73.34 & 73.88 & 61.11 & 61.01 & 64.0& & \multirow{1}{*}{\cite{gowal2018effectiveness}}&\multirow{1}{*}{67.96}&\multirow{1}{*}{50.51}\\
       &   & && 1&0 & 72.42 & 72.57 & 73.49 & 62.26 & 60.98 & 63.5 & & \multirow{1}{*}{\cite{xiao2018training}}&\multirow{1}{*}{79.73}&\multirow{1}{*}{59.55}\\
       &   & && 1&0.5 & 73.88 & 75.16 & 76.93 & \textbf{55.66} & \textbf{52.53} & \textbf{53.79} & &\multirow{1}{*}{\cite{dvijotham2018training}}&\multirow{1}{*}{73.33}&\multirow{1}{*}{51.36}\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0& \textbf{71.28} & \textbf{72.15} & \textbf{73.66} & 59.07 & 59.18 & 63.17 & & \multirow{1}{*}{\cite{wong2018scaling}}&\multirow{1}{*}{78.22}&\multirow{1}{*}{71.33}\\
       &    &   &   &  1 & 0  & 70.77  & 72.24  & 73.10  & 58.65  &  60.49 & 61.86  &   &  &   &   \\
       &  $\epsilon_\text{train}=8/255$  &   &   &  1 &  0.5 & 72.59  & 74.71  & 76.11  & 49.86  & 52.95  & 55.58  &   &  &   &   \\
    %   \midrule
    \cline{3-12}
 
    
        & $\epsilon_\text{test}=8/255$& \multirow{6}{*}{8 medium models} &\multirow{3}{*}{IBP}&0&0 & 72.75 & 73.23 & 73.82 & 59.23 & 65.96 & 66.35 & &&&\\
       &   & && 1&0 & 72.18 & 72.83 & 74.38 & 62.54 & 59.6 & 61.99 & & & &\\
       &   & && 1&0.5 & 74.84 & 75.59 & 97.93 & \textbf{51.71} & \textbf{54.41} & \textbf{54.12} & &&&\\
       \cline{4-12}&   & &\multirow{3}{*}{CROWN-IBP}&0&0& \textbf{70.79} & \textbf{71.17} & \textbf{72.29} & 57.82 & 58.68 & 59.73 & & & &\\
       &    &   &   &  1 & 0  & 70.51  & 71.96  & 72.82  &  57.87 & 59.98  & 59.16  &   &  &   &   \\
       &    &   &   &  1 &  0.5 & 73.48  &  74.69 & 76.66  & 49.40  & 53.56  & 52.05  &   &  &   &   \\
    %   \midrule

    \bottomrule[2pt]
    \end{tabular}
\begin{tablenotes}
\linespread{1.5}\selectfont
\item[1] {\Large For small $\epsilon$ IBP based methods tend to overfit on training set, thus we observe suboptimal verified errors on this table as we do not fine-tune hyperparameter for each individual setting. By adding explicit $\ell_1$ regularization, CROWN IBP can achieve \textbf{3.60\%} verified error at $\epsilon=0.1$ and \textbf{5.48\%} at $\epsilon=0.2$ (see Section~\ref{sec:small_eps}). Additionally, early stopping can also help achieve a better verified error; with early stopping the best verified errors achieved by CROWN-IBP are \textbf{3.55\%} at $\epsilon=0.1$ and \textbf{4.98\%} for $\epsilon=0.2$. See Figure~\ref{fig:epsschedulel}.}
\item[2] {\Large These models reported in \cite{gowal2018effectiveness} are trained at a larger $\epsilon_{\text{train}}$ than the $\epsilon$ used for evaluation. We always use the same $\epsilon$ for training and evaluation. \cite{gowal2018effectiveness} trained models with $\epsilon_{\text{train}}=0.2$ and evaluate them with $\epsilon=0.1$; they also trained models with $\epsilon_{\text{train}}=0.4$ and evaluate them with $\epsilon=0.3$ and $\epsilon=0.2$.}
%\item[3] {\Large Practically reproducible verified error is about 71\% - 72\%, matching our reported numbers for Natural-IBP. See \textcolor{blue}{\url{https://github.com/deepmind/interval-bound-propagation/issues/1\#issuecomment-492552237}}}
\item[3] {\Large We use $\beta=1$ for this setting.}

\end{tablenotes}
    \end{threeparttable}
}
%
    % \captionof{table}{Untargeted attack success rate against Mitsuba by transferring ``adversarial meshes'' generated by attacking a differentiable renderer targeting different classes.}
    %\vspace{-0.5cm}
\end{table}


==> bigtable1_before_before.tex <==
\begin{table}[ht]
\centering

    \caption{The robust and standard error of model trained on MNIST and CIFAR using different methods. Here we train 36 models using CROWN-IBP, pure-IBP and natural-IBP (with final $\kappa=$ 0 or 0.5). For each scenario, we pick 3 representative models among all models: the models with smallest, median, and largest robust error. We also report the standard error of these three selected models. }%\textcolor{blue}{the table looks like we only have 2 models, one large and one small. We should make sure other people do not misunderstand us.}
    \label{tbl:result} 
\adjustbox{max width=1.00\linewidth}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c||c|c|c}
    \toprule
        Dataset & Epsilon& Model Family & Method   & \multicolumn{3}{c|}{ Robust Test Error}& \multicolumn{3}{c|}{ Standard Test Error} & \multicolumn{3}{c}{The \textbf{Best} results in Literature} \\
        
        & & &  & best &median& worst & best & median & worst & Source & Rob. Err. & Std. Err. \\ 
        \midrule
      \multirow{32}{*}{\shortstack{MNIST}} &  \multirow{8}{*}{0.1}  & \multirow{4}{*}{10 small models}&Pure IBP & 0.0479 & 0.0574 & 0.0732 & 0.0148 & 0.0159 & 0.025 & \multirow{2}{*}{\cite{gowal2018effectiveness}($\epsilon_{train}=0.2$)}& \multirow{2}{*}{$0.0223$}&\multirow{2}{*}{$0.0106$} \\
       &   & & Natural IBP with final $\kappa=0$ &0.0487 & 0.0572 & 0.0724 & 0.0151 & 0.0134 & 0.0246 & & &\\
       &   & & Natural IBP with final $\kappa=0.5$ &0.0524 & 0.0595 & 0.0736 & 0.0141 & 0.0188 & \textbf{0.0187} &\multirow{2}{*}{\cite{xiao2018training}}& \multirow{2}{*}{$0.0440$}&\multirow{2}{*}{$0.0105$} \\
       &   & & CROWN-IBP &\textbf{0.0421} & \textbf{0.0518} & \textbf{0.068} & \textbf{0.0141} & \textbf{0.0183} & 0.0258& & &\\
    %   \midrule
    \cline{3-10}
 
    
        & & \multirow{4}{*}{8 large models} &Pure IBP & 0.059 & 0.0625 & 0.0782 & \textbf{0.0114} & 0.0112 & 0.0123&\multirow{2}{*}{\cite{wong2018scaling}}& \multirow{2}{*}{0.0367}&\multirow{2}{*}{0.0108} \\
       &   & & Natural IBP with final $\kappa=0$ & 0.0577 & 0.063 & 0.075 & 0.0121 & 0.0113 & 0.0134 & & &\\\cline{11-13}
       &   & & Natural IBP with final $\kappa=0.5$ & 0.0605 & 0.064 & 0.077 & 0.0119 & 0.0133 & 0.0124 &\multirow{2}{*}{\cite{dvijotham2018training}}& \multirow{2}{*}{0.0444}&\multirow{2}{*}{0.0120} \\
       &   & & CROWN-IBP & \textbf{0.0522} & \textbf{0.0563} & \textbf{0.0634} & 0.0119 & \textbf{0.0105} & \textbf{0.0103} & & &\\
    %   \midrule
    \cline{2-10}
    
    
    &  \multirow{8}{*}{0.2}  & \multirow{4}{*}{10 small models}&Pure IBP & 0.069 & 0.0824 & 0.1267 & 0.0193 & 0.0276 & 0.0414 &\multirow{4}{*}{\cite{gowal2018effectiveness}($\epsilon_{train}=0.4$)}& \multirow{4}{*}{$0.0448$}&\multirow{4}{*}{$0.0166$} \\
       &   & & Natural IBP with final $\kappa=0$ & 0.0684 & 0.0816 & 0.1292 & 0.0201 & 0.0256 & 0.0393 & & &\\
       &   & & Natural IBP with final $\kappa=0.5$ &0.0731 & 0.0871 & 0.1354 & \textbf{0.0162} & 0.0236 & \textbf{0.0322} &&&\\
       &   & & CROWN-IBP &\textbf{0.0611} & \textbf{0.0729} & \textbf{0.1197} & 0.0193 & \textbf{0.023} & 0.0386 & & &\\
    %   \midrule
    \cline{3-13}
 
    
        & & \multirow{4}{*}{8 large models} &Pure IBP & 0.0756 & 0.086 & 0.098 & 0.0196 & 0.0219 & 0.0139 &\multirow{4}{*}{\cite{xiao2018training}}& \multirow{4}{*}{$0.1021$}&\multirow{4}{*}{$0.0190$} \\
       &   & & Natural IBP with final $\kappa=0$ &0.0826 & 0.0872 & 0.0984 & 0.0145 & 0.0173 & \textbf{0.0131} & & &\\
       &   & & Natural IBP with final $\kappa=0.5$ & 0.0842 & 0.089 & 0.1009 & 0.0176 & 0.0142 & 0.0153 & & &\\
       &   & & CROWN-IBP & \textbf{0.0606} & \textbf{0.0642} & \textbf{0.0764} & \textbf{0.0109} & \textbf{0.0133} & 0.0136 & & &\\
    %   \midrule
    \cline{2-13}
       
       
       

       
       
    &  \multirow{8}{*}{0.3}  & \multirow{4}{*}{10 small models}&Pure IBP & 0.1054 & 0.1202 & 0.2047 & 0.0278 & \textbf{0.0331} & 0.0607 &\multirow{2}{*}{\cite{gowal2018effectiveness}($\epsilon_{train}=0.4$)}&\multirow{2}{*}{0.0805}&\multirow{2}{*}{0.0166}\\
       &   & & Natural IBP with final $\kappa=0$ &0.0996 & 0.1209 & 0.21 & 0.027 & 0.0348 & 0.0668 & & &\\\cline{11-13}
       &   & & Natural IBP with final $\kappa=0.5$ & 0.1037 & 0.1278 & 0.2199 & \textbf{0.0211} & 0.0344 & \textbf{0.0519}& \multirow{3}{*}{\cite{wong2018scaling}}&\multirow{3}{*}{0.4310}&\multirow{3}{*}{0.1487}\\
       &   & & CROWN-IBP & \textbf{0.0887} & \textbf{0.1129} & \textbf{0.1683} & 0.0243 & 0.0362 & 0.0726 & & &\\
    %   \midrule
    \cline{3-10}
 
    
        & & \multirow{4}{*}{8 large models} &Pure IBP & 0.1043 & 0.1083 & 0.1199 & 0.0201 & 0.0238 & 0.0329 &&&\\\cline{11-13}
       &   & & Natural IBP with final $\kappa=0$ & 0.1074 & 0.1173 & 0.1216 & 0.0217 & 0.0246 & \textbf{0.016} &\multirow{3}{*}{\cite{xiao2018training}}&\multirow{3}{*}{0.1932}&\multirow{3}{*}{0.0267}\\
       &   & & Natural IBP with final $\kappa=0.5$ & 0.1123 & 0.1171 & 0.124 & 0.0172 & 0.0209 & 0.0163 & & &\\
       &   & & CROWN-IBP &\textbf{0.0746} & \textbf{0.0847} & \textbf{0.0857} & \textbf{0.0148} & \textbf{0.0152} & 0.0199 & & &\\
    %   \midrule
    \cline{2-13}
       
        
       
       
       
       
    &  \multirow{8}{*}{0.4}  & \multirow{4}{*}{10 small models}&Pure IBP& 0.1672 & 0.1889 & 0.3742 & 0.042 & 0.054 & 0.0963 &\multirow{8}{*}{\cite{gowal2018effectiveness}}&\multirow{8}{*}{0.1488}&\multirow{8}{*}{0.0166}\\
       &   & & Natural IBP with final $\kappa=0$ & 0.161 & 0.1875 & 0.353 & 0.038 & 0.0493 & 0.1132 & & &\\
       &   & & Natural IBP with final $\kappa=0.5$ & 0.1654 & 0.1914 & 0.3542 & \textbf{0.034} & \textbf{0.0365} & \textbf{0.0754} & & &\\
       &   & & CROWN-IBP &\textbf{0.1538} & \textbf{0.1857} & \textbf{0.2456} & 0.0361 & 0.0483 & 0.0846 & & &\\
    %   \midrule
    \cline{3-10}
 
    
        & & \multirow{4}{*}{8 large models} &Pure IBP & 0.1517 & 0.1654 & 0.1898 & 0.0283 & 0.0379 & 0.0491 &&&\\
       &   & & Natural IBP with final $\kappa=0$ &0.1563 & 0.1606 & 0.1711 & 0.0293 & 0.034 & 0.0375 & & &\\
       &   & & Natural IBP with final $\kappa=0.5$ & 0.1574 & 0.1642 & 0.1798 & \textbf{0.0235} & \textbf{0.0231} & \textbf{0.0315} & & &\\
       &   & & CROWN-IBP &\textbf{0.1296} & \textbf{0.1343} & \textbf{0.1425} & 0.0276 & 0.0285 & 0.0336 & & &\\
       
 
       
       
       
       
    \midrule
    \multirow{16}{*}{\shortstack{CIFAR}} &  \multirow{8}{*}{2/255}  & \multirow{4}{*}{10 small models}&Pure IBP & 0.5469 & 0.5784 & 0.6058 & 0.4059 & 0.4551 & 0.5138 &\multirow{2}{*}{\cite{gowal2018effectiveness}}&\multirow{2}{*}{0.4998}&\multirow{2}{*}{0.2984}\\
       &   & & Natural IBP with final $\kappa=0$ & 0.5456 & 0.5842 & 0.6069 & 0.4032 & 0.4742 & 0.5073 & & &\\\cline{11-13}
       &   & & Natural IBP with final $\kappa=0.5$ & 0.5689 & 0.6066 & 0.6358 & \textbf{0.3428} & \textbf{0.3928} & \textbf{0.4803}& \multirow{3}{*}{\cite{wong2018scaling}}&\multirow{3}{*}{0.4611}&\multirow{3}{*}{0.3172}\\
       &   & & CROWN-IBP & \textbf{0.5246} & \textbf{0.5755} & \textbf{0.6067} & 0.3911 & 0.4676 & 0.5086 & & &\\
    %   \midrule
    \cline{3-10}
 
    
        & & \multirow{4}{*}{8 large models} &Pure IBP & 0.5547 & 0.5641 & 0.5854 & 0.4159 & 0.4433 & 0.4654 & & &\\\cline{11-13}
       &   & & Natural IBP with final $\kappa=0$ & 0.5551 & 0.5674 & 0.5785 & 0.4241 & 0.4371 & 0.4474 &\multirow{3}{*}{\cite{xiao2018training}}&\multirow{3}{*}{0.5407}&\multirow{3}{*}{0.3888}\\
       &   & & Natural IBP with final $\kappa=0.5$ & 0.5705 & 0.597 & 0.6025 & \textbf{0.3477} & \textbf{0.358} & \textbf{0.3895} & & &\\
       &   & & CROWN-IBP & \textbf{0.5252} & \textbf{0.539} & \textbf{0.5605} & 0.3934 & 0.4007 & 0.4357 & & &\\
    %   \midrule
    \cline{2-13}
    
    
    &  \multirow{8}{*}{8/255}  & \multirow{4}{*}{10 small models}&Pure IBP & 0.7207 & 0.7334 & 0.7388 & 0.6111 & 0.6101 & 0.64& \multirow{2}{*}{\cite{gowal2018effectiveness}}&\multirow{2}{*}{0.6796}&\multirow{2}{*}{0.5051}\\
       &   & & Natural IBP with final $\kappa=0$ & 0.7242 & 0.7257 & 0.7349 & 0.6226 & 0.6098 & 0.635 & & &\\\cline{11-13}
       &   & & Natural IBP with final $\kappa=0.5$ & 0.7388 & 0.7516 & 0.7693 & \textbf{0.5566} & \textbf{0.5253} & \textbf{0.5379} &\multirow{2}{*}{\cite{xiao2018training}}&\multirow{2}{*}{0.7973}&\multirow{2}{*}{0.5955}\\
       &   & & CROWN-IBP & \textbf{0.7128} & \textbf{0.7215} & \textbf{0.7366} & 0.5907 & 0.5918 & 0.6317 & & &\\
    %   \midrule
    \cline{3-13}
 
    
        & & \multirow{4}{*}{8 large models} &Pure IBP & 0.7275 & 0.7323 & 0.7382 & 0.5923 & 0.6596 & 0.6635 &\multirow{2}{*}{\cite{wong2018scaling}}&\multirow{2}{*}{0.7822}&\multirow{2}{*}{0.7133}\\
       &   & & Natural IBP with final $\kappa=0$ & 0.7218 & 0.7283 & 0.7438 & 0.6254 & 0.596 & 0.6199 & & &\\\cline{11-13}
       &   & & Natural IBP with final $\kappa=0.5$ & 0.7484 & 0.7559 & 0.9793 & \textbf{0.5171} & \textbf{0.5441} & \textbf{0.5412} &\multirow{2}{*}{\cite{dvijotham2018training}}&\multirow{2}{*}{0.7333}&\multirow{2}{*}{0.5136}\\
       &   & & CROWN-IBP & \textbf{0.7079} & \textbf{0.7117} & \textbf{0.7229} & 0.5782 & 0.5868 & 0.5973 & & &\\
    %   \midrule

    \bottomrule
    \end{tabular}
}
    % \captionof{table}{Untargeted attack success rate against Mitsuba by transferring ``adversarial meshes'' generated by attacking a differentiable renderer targeting different classes.}
    \vspace{-0.5cm}
\end{table}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

